Cloth2Tex: A Customized Cloth Texture Generation Pipeline for 3D Virtual Try-On

Fabricating and designing 3D garments has become extremely demanding with the increasing need for synthesizing realistic dressed persons for a variety of applications, e.g. 3D virtual try-on, digitalization of 2D clothes into 3D apparel, and cloth animation. It thus necessitates a simple and straightforward pipeline to obtain high-quality texture from simple input, such as 2D reference images. Since traditional warping-based texture generation methods require a significant number of control points to be manually selected for each type of garment, which can be a time-consuming and tedious process. We propose a novel method, called Cloth2Tex, which eliminates the human burden in this process. Cloth2Tex is a self-supervised method that generates texture maps with reasonable layout and structural consistency. Another key feature of Cloth2Tex is that it can be used to support high-fidelity texture inpainting. This is done by combining Cloth2Tex with a prevailing latent diffusion model. We evaluate our approach both qualitatively and quantitatively and demonstrate that Cloth2Tex can generate high-quality texture maps and achieve the best visual effects in comparison to other methods. Project page: tomguluson92.github.io/projects/cloth2tex/

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> utils.tex <==
\definecolor{DeltaColor}{rgb}{0.039,0.73,0.71}
\definecolor{SigmaColor}{rgb}{0.98,0.45,0.0}
\definecolor{AlphaColor}{rgb}{0,0,0.8}
\definecolor{BetaColor}{rgb}{0.8,0,0.8}
\definecolor{GammaColor}{rgb}{0.514,0.34,0.224}
\definecolor{EpsilonColor}{rgb}{0.353,0.725,0.906}
\definecolor{GreenColor}{rgb}{0.137,0.573,0.565}
\definecolor{RedColor}{rgb}{0.949,0.275, 0.224}
\definecolor{BlueColor}{rgb}{0.0,0.0, 0.99}
\definecolor{citecolor}{HTML}{0071bc}

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\newcommand{\algrule}[1][.2pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip}
\renewcommand{\arraystretch}{1.0}

\newcommand{\projectURL}{\href{https://dart2022.github.io/}{\tt{dart2022.github.io}}}

\setlength{\extrarowheight}{1pt}

\newcommand{\daiheng}[1]{{\color{BetaColor} Daiheng: #1 }}
\newcommand{\xuchen}[1]{{\color{EpsilonColor} Xuchen: #1 }}
\newcommand{\todo}[1]{{\color{EpsilonColor} TODO: #1 }}

\newcommand{\xindi}[1]{{\color{SigmaColor} Xindi: #1 }}

% \newcommand{\update}[1]{{\color{DeltaColor} #1}}
\newcommand{\update}[1]{{\color{Black} #1}}
\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}


% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

\newcommand{\method}{Cloth2Tex\xspace}

\newcommand{\xmark}{\textcolor{RedColor}{\ding{55}}\xspace}
\newcommand{\cmark}{\textcolor{GreenColor}{\ding{51}}\xspace}

\newcommand{\qheading}[1]{\noindent\mbox{\textbf{#1}}}
% \newcommand{\etc}{\mbox{etc}\xspace}
% \newcommand{\etal}{\mbox{et al.}\xspace}
% \newcommand{\ie}{\mbox{i.e.}\xspace}
% \newcommand{\eg}{\mbox{e.g.}\xspace}
% \newcommand{\wrt}{\mbox{w.r.t.}\xspace}

\newcommand{\texNum}{\mbox{325}\xspace}
\newcommand{\acsNum}{\mbox{50}\xspace}

% shline
\newlength\savewidth\newcommand\shline{\noalign{\global\savewidth\arrayrulewidth
\global\arrayrulewidth 2pt}\hline\noalign{\global\arrayrulewidth\savewidth}}
\newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize}

% automatic add fig. tab.
\newcommand{\colorRef}[1]{\textcolor{RedColor}{#1}}
\crefname{figure}{\colorRef{Fig.}}{\colorRef{Figs.}}
\Crefname{figure}{\colorRef{Figure}}{\colorRef{Figures}}
\crefname{section}{\colorRef{Sec.}}{\colorRef{Secs.}}
\Crefname{section}{\colorRef{Section}}{\colorRef{Sections}}
\Crefname{table}{\colorRef{Table}}{\colorRef{Tables}}
\crefname{table}{\colorRef{Tab.}}{\colorRef{Tabs.}}
